Adaptive LSQR Preconditioning from One Small Sketch

We propose APLICUR, an adaptive preconditioning framework for large-scale linear least-squares (LLS) problems. Using a single small sketch computed once at initialization, APLICUR incrementally refines a CUR-based preconditioner throughout the Krylov solve, interleaving preconditioning with iteration. This enables early convergence without the need to construct a costly high-quality preconditioner upfront. With a modest sketch dimension (typically 5 - 250), largely independent of both the problem size and numerical rank, APLICUR achieves convergence guarantees that are likewise independent of the sketch size. The method is applicable to general matrices without structural assumptions (e.g. need not be heavily overdetermined) and is well suited to large, sparse, or numerically low-rank problems. We conduct extensive numerical studies to examine the behavior of the proposed framework and guide the effective algorithmic design choices. Across a range of test problems, \mainalg{} achieves competitive or improved time-to-accuracy performance compared with established randomized preconditioners, including Blendenpik and Nystr\"om PCG, while maintaining low setup cost and robustness across problem regimes.

==> appendices_old.tex <==
\section{Appendices}
This appendix provides supplementary material supporting the main text, including proofs of the theoretical results, technical details for efficient implementation (such as factorization strategies, parameter choices, and practical considerations), and additional numerical results.
\subsection{Theoretical Results}

\subsubsection{Proof of \cref{thm:conditionnumberbound}}\label{proof:conditionnumberbound}

\begin{proof}
Let $\mtx{\widehat A} = \mtx{\widehat U \widehat \Sigma \widehat V^\top}$ be a rank-$\ell$ approximation of $\mtx{A}$, and define the error $\mtx{E} := \mtx{A} - \mtx{\widehat A}$. Recall that the regularized augmented matrix is
\[
\mtx{A}_\mu = \begin{bmatrix} \mtx{A} \\ \mu \mtx{I} \end{bmatrix}.
\]

We analyze first the idealized system based on $\mtx{\widehat A}$, and then account for the perturbation.

\paragraph{Step 1: Idealized system}

Define
\[
\mtx{\widehat A}_\mu := \begin{bmatrix} \mtx{\widehat A} \\ \mu \mtx{I} \end{bmatrix}.
\]
Let
\[
\mtx{\widehat\Sigma}_{\mathrm{full}} =
\begin{bmatrix}
\mtx{\widehat\Sigma} & \\
& \mtx{0}
\end{bmatrix}, 
\quad
\mtx{\widehat V}_{\mathrm{full}} = [\mtx{\widehat V} \ \mtx{\widehat V}_\perp].
\]

By construction of the preconditioner,
\begin{align*}
\mtx{P}_\mu^{-\top}\mtx{\widehat A}_\mu^\top \mtx{\widehat A}_\mu \mtx{P}_\mu^{-1}
&= \mtx{P}_\mu^{-\top}(\mtx{\widehat A}^\top \mtx{\widehat A} + \mu^2 \mtx{I})\mtx{P}_\mu^{-1} \\
&= \mtx{\widehat V}_{\mathrm{full}}
\begin{bmatrix}
\widehat\sigma^2 \mtx{I}_\ell & \\
& \mu^2 \mtx{I}
\end{bmatrix}
\mtx{\widehat V}_{\mathrm{full}}^\top.
\end{align*}

% \begin{align*}
%         \mtx{P}_\mu^{-\top}\mtx{\widehat{A}}_\mu^\top \mtx{\widehat{A}}_\mu \mtx{P}_\mu^{-1} = \mtx{P}_\mu^{-\top}(\mtx{\widehat{A}}^\top \mtx{\widehat{A}}+\mu^2 \mtx{I_n} ) \mtx{P}_\mu^{-1}= \mtx{P}_\mu^{-\top}\Vhat_{full} (\Lhat_{full}^2 + \mu^2\mtx{I_n})\Vhat_{full}^\top\mtx{P}_\mu^{-1} \\
%         =\Vhat_{full}\begin{bmatrix} \svhat(\Lhat^2+\mu^2\mtx{I_\l})^{-1/2}&\\
%             & \mtx{I_{n-\l}} \end{bmatrix}
%             \begin{bmatrix} \Lhat^2+\mu^2\mtx{I_\l}&\\
%             & \mu^2\mtx{I_{n-\l}} \end{bmatrix}  
%             \begin{bmatrix} \svhat(\Lhat^2+\mu^2\mtx{I_\l})^{-1/2}&\\
%             & \mtx{I_{n-\l}} \end{bmatrix}
%             \Vhat_{full}^\top\\
%         = \Vhat_{full}\begin{bmatrix}  \svhat^2&\\
%             & \mu^2\mtx{I_{n-\l}} \end{bmatrix}
%             \Vhat_{full}^\top
%     \end{align*}

Hence, the singular values of $\mtx{\widehat A}_\mu \mtx{P}_\mu^{-1}$ are
\[
\sqrt{\widehat\sigma^2 + \mu^2} \quad (\ell \text{ times}), 
\qquad
\mu \quad (n-\ell \text{ times}).
\]

In other words, $\mtx{P}_\mu^{-1}$ rescales only the $\mtx{\widehat V}$-subspace and acts as an isometry on its orthogonal complement.

\paragraph{Step 2: Perturbation}

Write
\[
\mtx{A}_\mu \mtx{P}_\mu^{-1}
= \mtx{\widehat A}_\mu \mtx{P}_\mu^{-1}
+ \underbrace{\begin{bmatrix} \mtx{E} \\ \mtx{0} \end{bmatrix} \mtx{P}_\mu^{-1}}_{:=\mtx{\Delta}}.
\]

Using $\svhat \le \sqrt{\widehat\sigma_\ell^2 + \mu^2}$, we have $\|\mtx{P}_\mu^{-1}\|_2 \le 1$, hence obtain
$\|\mtx{\Delta}\|_2 \le \|\mtx{E}\|_2$.
Applying Weyl’s inequality,
\begin{align*}
\sigma_{\max}(\mtx{A}_\mu \mtx{P}_\mu^{-1})
&\le \sqrt{\widehat\sigma^2 + \mu^2} + \|\mtx{E}\|_2,\\
\sigma_{\min}(\mtx{A}_\mu \mtx{P}_\mu^{-1})
&\ge \mu - \|\mtx{E}\|_2.
\end{align*}

\paragraph{Step 3: Condition number}

If $\|\mtx{E}\|_2 < \mu$, then
\[
\kappa(\mtx{A}_\mu \mtx{P}_\mu^{-1})
\le \frac{\sqrt{\widehat\sigma^2 + \mu^2} + \|\mtx{E}\|_2}{\mu - \|\mtx{E}\|_2}.
\]
\end{proof}

\subsubsection{Proof of \cref{thm:cvgbound_chebyshev}}\label{proof:cvgbound_chebyshev}
\begin{theorem}\label{thm:cvgbound_chebyshev}
    Let $\mtx{A}$ be a $m \times n$ matrix and $\vct{b} \in \mathbb{R}^n$. Let $\vct{r_k}:= \mtx{Ax_k}-\vct{b}$ be the residual after the $k$-th LSQR iteration and $\mtx{A} = \mtx{U\Sigma V}^\top$ be the SVD decomposition with $\mtx{\Sigma} = \text{diag}(\sigma_1, \ldots, \sigma_n)$. Then,
    \begin{align}
        \|\mtx{U}^\top \vct{r_k}\|_2 \leq 2 \left(\frac{\kappa(\mtx{A})-1}{\kappa(\mtx{A})+1}\right)^k \|\mtx{U}^\top \vct{r_0} \|_2,
    \end{align}
    where $\kappa(\mtx{A}) = \sigma_1/\sigma_n$ is the condition number of $\mtx{A}$.
\end{theorem}
\yn{ I'm happy for you to keep this derivation in your transfer, but not for SISC (and probably not even for arXiv).}
\begin{proof}
    Starting from an initial guess $\vct{x_0}$, LSQR  finds the $k$-th iterate $\vct{x}_k$ the affine Krylov subspace $$\mathcal{K}_k^{\vct{x_0}} := \vct{x_0} + \mathcal{K}_k(\mtx{A^\top A}, \mtx{A^\top}\vct{r_0}),$$ to minimize the residual norm $\|\mtx{A}\vct{x}_k-\vct{b}\|_2$ over this space.
    
    Given that $\vct{x_\ast} = \mtx{V\Sigma^\dagger U^\top b}$, we have $$\|\vct{x} - \vct{x_\ast}\|_{\mtx{A^\top A}} = \|\mtx{\Sigma V^\top}(\vct{x} - \vct{x_\ast})\|_2 = \|\mtx{U}^\top (\mtx{A}\vct{x} - \vct{b})\|_2.$$
    Hence, the projected residual at iteration $k$ can be written as
    \begin{align}
        \|\mtx{U^\top}(\mtx{A}\vct{x}_k - \vct{b})\|_2^2 
        &= \min_{\vct{x} \in \mathcal{K}_k^{\vct{x_0}}} \|\vct{x} - \vct{x_\ast}\|_{\mtx{A^\top A}}^2 \notag\\
        &= \min_{p_{k-1} \in \mathcal{P}_{k-1}}\|\vct{x_0} + p_k(\mtx{A^\top A})\mtx{A^\top}(\vct{b} - \mtx{A x_0}) - \vct{x_\ast}\|_{\mtx{A^\top A}}^2 \notag\\
        &=\min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}} \|p_k(\mtx{A^\top} \mtx{A})(\vct{x_0} - \vct{x_\ast})\|_{\mtx{A^\top A}}^2 \notag\\
        &=\min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}} \|\mtx{V} p_k(\mtx{\Sigma}^2)\mtx{V^\top}(\vct{x_0} - \vct{x_\ast})\|_{\mtx{A^\top A}}^2 \notag\\
        &= \min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}} \sum_i \sigma_i^2 (\vct{v}_i^\top (\vct{x_0}-\vct{x}_\ast))^2 p_k(\sigma_i^2)^2\\
        &\leq \min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}}  \max_j p_k(\sigma_j^2)^2  \sum_i \left(\sigma_i \vct{v_i}^\top(\vct{x_0} - \vct{x_\ast})\right)^2 \notag\\
        &= \min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}} \max_j p_k(\sigma_j^2)^2 \cdot \|\mtx{x_0} - \vct{x_\ast}\|_{\mtx{A^\top A}}^2. \notag \\
        &= \|\mtx{U^\top}(\mtx{Ax_0} - \vct{b})\|_2^2 \cdot \min_{\substack{p_k \in \mathcal{P}_k\\p_k(0) = 1}} \max_j p_k(\sigma_j^2)^2. \notag
    \end{align}

    The minimax problem is bounded by scaled Chebyshev polynomials, giving
    A well-known bound for the last term is given by the shifted and scaled Chebyshev polynomial $T_k$:\jh{Add reference that the Chebyshev polynomial is the optimal solution to the LHS below}
    \begin{align}\label{eq:convergencebound_singleinterval}
        \min_{\substack{p_{k} \in \mathcal{P}_k\\p_k(0) = 1}}\max_{z \in [\sigma_n^2,\sigma_1^2]} |p_k(z)| 
        = \max_{z \in [\sigma_n^2,\sigma_1^2]} \left|\frac{T_k(\frac{2z-\sigma_1^2 - \sigma_n^2}{\sigma_1^2 - \sigma_n^2})}{T_k(\frac{\sigma_1^2 + \sigma_n^2}{\sigma_1^2 - \sigma_n^2})}\right| 
        \leq 2 \left(\frac{\kappa(\mtx{A})-1}{\kappa(\mtx{A})+1}\right)^{k}
    \end{align}
\end{proof}

\subsubsection{Gap-aware LSQR convergence bound}\label{app:twointervalbound} 
\label{proof:cvgbound_disjoint}

The classical Chebyshev bound depends only on the global condition number $\kappa(\mtx{A})$ and is therefore is often pessimistic for systems with clustered spectra.

Assume that the dominant singular values lie in a narrow interval:
\[
\sigma_1^2, \ldots, \sigma_\ell^2 \in [\svhat^2 - \varepsilon,\ \svhat^2 + \varepsilon],
\]
while the remaining singular values lie below $\sigma_{\ell+1}$.
Thus, the spectrum is contained in two disjoint intervals:
\[
[\sigma_n^2, \sigma_{\ell+1}^2]
\cup
[\sigma_\ell^2, \sigma_1^2].
\]

To exploit this structure, we bound the LSQR residual via polynomial approximation over the union
\[
\mathcal{S}
:=
[a,b] \cup [c,d] \supseteq [\sigma_n^2, \sigma_{\ell+1}^2]
\cup
[\sigma_\ell^2, \sigma_1^2],
\]
where both intervals of $\mathcal{S}$ have equal length $w$.

\begin{lemma}[\cref{thm:cvgbound_disjoint}]
Under the above assumptions, the LSQR residual at $k$-th iterate $\vct{x}_k$ satisfies
\[
\|\mtx{U}^\top(\mtx{A} \vct{x}_k - \vct{b})\|_2
\le
\left(\frac{\sqrt{C}-1}{\sqrt{C}+1}\right)^{\lfloor k/2 \rfloor},
\]
where $\mtx{U}$ is the left singular vector matrix of $\mtx{A}$ and
\[
C
=
\kappa_{\ell+1}^2 + \frac{w}{\sigma_n^2}.
\]
\end{lemma}

\begin{proof}[Proof of \cref{thm:cvgbound_disjoint}]
    
    Define $w_1 := \sigma_1^2 - \sigma_\l^2$ and $w_2 := \sigma_{\l+1}^2 - \sigma_n^2$, and let $w := \max\{w_1, w_2\}$. Then, take
    \begin{align}
        a:= \sigma_n^2, \quad b:= \sigma_n^2 + w > \sigma_{\l+1}^2,
        \quad c:= \sigma_\l^2, \quad d:= \sigma_\l^2 + w > \sigma_{1}^2.
    \end{align}
    This constructs a union of two disjoint intervals of equal length $w$: $$\mathcal{S} := [a, b] \cup [c, d] \supseteq [\sigma_n^2, \sigma_{\l+1}^2] \cup [\sigma_\l^2, \sigma_1^2].$$
    
    We introduce the quadratic polynomial $$q_2(\lambda) = 1 + \frac{2(\lambda - b)(\lambda - c)}{ad - bc}$$ which maps both intervals of $\mathcal{S}$ to $[-1,1]$, each monotonically (this is possible because the intervals have equal length~\cite{ashby1988polynomial}). Then, consider the polynomial
    \begin{align}
        p_k(z) = \frac{T_{\lfloor{\frac{k}{2}}\rfloor}(q_2(z))}{T_{\lfloor{\frac{k}{2}}\rfloor}(q_2(0))}.
    \end{align}
    By the boundedness property of the ordinary Chebyshev polynomial on $[-1,1]$, we obtain the bound 
    \begin{align}
        \max_{z \in \mathcal{S}} |p_k(z)| \leq \frac{1}{\left|T_{\lfloor{\frac{k}{2}}\rfloor}\left(\frac{bc + ad}{bc - ad}\right)\right|} \leq \left(\frac{\sqrt{\frac{bc}{ad}}-1}{\sqrt{\frac{bc}{ad}}+1}\right)^{\lfloor{\frac{k}{2}}\rfloor},
    \end{align}
    where the equal length property of the intervals ensures $bc > ad$.

    To bound $\frac{bc}{ad}$, we introduce $\eta := |w_1 - w_2| < \max\{w_1, w_2\}$ and derive
    \begin{align*}
        \frac{bc}{ad} 
        &\leq \frac{\sigma_{\l+1}^2 + \eta}{\sigma_n^2}\cdot\frac{\sigma_\l^2}{\sigma_1^2} 
        \leq \frac{\sigma_{\l+1}^2 + \eta}{\sigma_n^2} 
        < \kappa_{\l+1}^2 + \frac{\max\{w_1, w_2\}}{\sigma_n^2}\\
        &\leq \kappa_{\l+1}^2 + \max\left\{\frac{2\eps}{\sigma_n^2}, \kappa_{\l+1}^2 - 1\right\}.
    \end{align*}
\end{proof}

\begin{remark}
The bound depends only on $\kappa_{\ell+1}$ and the cluster widths, rather than the global condition number $\kappa( \mtx A)$. Hence, large spectral gaps do not degrade convergence once clustering is achieved.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{CUR Approximation Details}\label{app:cur_details}
There exists a wide variation of CUR approximations, which differ in several aspects: (1) row and column selection, (2) the construction of the core matrix $\mtx{U}$, and (3) the choice of target rank $\l$.

\subsubsection{Row and column selection}

Selecting appropriate row and column is crucial to the quality of the CUR approximation. Existing methods are broadly classified into two categories. The first consists of sampling-based approaches, which draw indices according to specific probability distributions, including leverage score \cite{drineas2008relative, mahoney2009cur}, uniform \cite{chiu2013sublinear}, volume \cite{deshpande2006matrix, deshpande2010efficient, cortinovis2020low}, determinantal point process (DPP) \cite{derezinski2021determinantal}, K-means++ \cite{oglic2017nystrom}, and BSS sampling \cite{batson2014twice, boutsidis2014near}. The second category uses pivoting-based approaches, where strategies such as column-pivoted QR (CPQR) \cite{golub2013matrix}, LU with partial or complete pivoting \cite{trefethen2022numerical, dong2023simpler}, and strong rank-revealing factorisations \cite{hong1992rank, gu1996efficient, pan2000existence}  identify informative rows and columns via the permutation vectors generated during factorisation.

\jh{Maybe we can add separate subsection on sketching techniques}
For large matrices, directly selecting informative indices from $\mtx{A}$ can be costly, so randomized techniques construct a smaller "sketch" $\mtx{X}$ that preserves sufficient information for selection \cite{halko2011finding, drineas2008relative, voronin2017efficient, duersch2020randomized, dong2023simpler}. Given a matrix $\mtx{A} \in \mathbb{R}^{m \times n}$, a sketch is formed by multiplying $\mtx{A}$ with a random embedding matrix $\mtx{S}$, yielding $\mtx{X} = \mtx{SA}$ (or $\mtx{X} = \mtx{AS}$ depending on whether rows or columns are being sketched). Several sketching techniques are commonly used, including Gaussian sketch \cite{halko2011finding, indyk1998approximate, martinsson2020randomized, woodruff2014sketching}, where $\mtx{S}$ is a Gaussian matrix, or subsampled randomised trigonometric transform (SRTT) \cite{ailon2009fast, halko2011finding, martinsson2020randomized, woolfe2008fast, tropp2011improved, rokhlin2008fast}, hashing embedding \cite{cartis2021hashing}, or sparse sign embedding \cite{martinsson2020randomized, nelson2013osnap, kane2014sparser, woodruff2014sketching, clarkson2017low, meng2013low}. It is known that sketching incurs only minor losses in accuracy \cite{halko2011random}.
\jh{Sketching not only is helpful for large scale matrices, but it also helps CPQR and LUPP to be robust to adversarial inputs in practice (Remark 6 of\cite{trefethen1990average}).}

\subsubsection{Choice of the core matrix}

There are largely two different choices for the core matrix $\mtx{U}$, namely CUR with Best Approximation (CUR-BA) and CUR with Cross Approximation (CUR-CA). CUR-BA chooses $\mtx{U} = \min_{\mtx{Z}} \|\mtx{A} - \mtx{CZR}\|_F =\mtx{C}^\dagger \mtx{A} \mtx{R}^\dagger$, where the theoretical bound that is at most a factor $\sqrt{2\l+2}$ larger than the best rank-$\l$ approximation error can be found in \cite{sorensen2016deim, dong2023simpler, osinsky2023close}. CUR-CA is rather choosing $\mtx{U}$ to be the pseudoinverse of the intersection of the selected columns and rows, namely $\mtx{U} = \mtx{A}(\vct{I}, \vct{J})^\dagger$. This type of construction requires the evaluation of $\mtx{A}$ only along the cross of $\l$ rows and $\l$ columns, which is particularly advantageous when the access to full matrix $\mtx{A}$ is not readily available. However, CUR-CA comes with the drawback that $\mtx{A}(\vct{I},\vct{J})$ can be (nearly) singular, leading to unfavorable approximation error due to the numerical instability in computing (pseudo)inverse \cite{dong2023simpler, martinsson2020randomized, sorensen2016deim}. For this reason, techniques like $\varepsilon$-pseudoinverse variant \cite{chiu2013sublinear} or oversampling \cite{park2025accuracy} are proposed to avoid numerical instability. 

\jh{CUR-CA bounds from volume sampling\cite{cortinovis2020low, zamarashkin2018existence} || Other references 
\cite{deshpande2006matrix} || polynomial bound for cross approximation in the maximum norm when choosing I, J such that the volume of A(I,J) is maximal \cite{goreinov2001maximal}}

Despite these concerns, we adopt CUR-CA due to its low computational cost and its suitability for constructing lightweight preconditioners. In our setting, stability is maintained through oversampled sketching, which mitigate ill-conditioning in $\mtx{A}(\vct{I}, \vct{J})$. The full procedure is given in \cref{alg:cur}. The total computational cost is $\mathcal{O}((m+n+\l)\l^2)$. Specifically, forming $\mtx{C}$ via randomized LUPP on $\mtx{Y}^\top \in \F^{n \times d}$ costs $\mathcal{O}(nd^2)$, while forming $\mtx{R}$ via LUPP on $\mtx{C} \in \F^{m \times \l}$ costs $\mathcal{O}(m\l^2)$.


\begin{algorithm}
    \caption{Sketched CUR with Cross Approximation using LUPP \cite{dong2023simpler}}\label{alg:cur}
    \begin{algorithmic}[1]
        \Require{$\mtx{A} \in \F^{m \times n}$, target rank $\ell$}
        \Ensure Row indices $\vct{I}$, column indices $\vct{J}$
        \Statex
        \Function{CURApproximation}{$\mtx{A}, \ell$}
            \State $\mtx{S} \gets \texttt{sparsesign}(\lfloor{1.1\l}\rfloor, m, 8)$ \Comment{sparse sign embedding with $\xi = 8$}
            \State $[\sim, \sim, \vct{P}_{col}] \gets \texttt{lu}((\mtx{S}\mtx{A})^\top, \texttt{`vector'})$
            \Comment{LUPP of $(\mtx{S}\mtx{A})^\top$}
            \State $\vct{J} \gets \vct{P}_{col}(1:\ell)$ \Comment{select $\ell$ columns}
            \State $\mtx{C} \gets \mtx{A}(:,\vct{J})$

            \State $[\sim, \sim, \vct{P}_{row}] \gets \texttt{lu}(\mtx{C}, \texttt{`vector'})$
            \Comment{LUPP of $\mtx{C}$}
            \State $\vct{I} \gets \vct{P}_{row}(1:\ell)$
            \Comment{select $\ell$ rows}
            \State $\mtx{R} \gets \mtx{A}(\vct{I}, :)$
            \State $\mtx{U} \gets \mtx{A}(\vct{I}, \vct{J})^\dagger$ 
            \Comment{default QR, improved efficiency with LU}
            
            \State \Return $\mtx{C}, \mtx{U}, \mtx{R}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\begin{theorem}[Theorem 2 in \cite{osinsky2023close}]\label{thm:curosinsky}
    Let $\mtx{A}, \mtx{Z} \in \mathbb{R}^{m \times n}$, $\text{rank}(\mtx{Z}) = \l$ given. Then in $\mathcal{O}(mn\l)$ operations it is possible to find rows $\mtx{R} \in \mathbb{R}^{\l \times n}$ and columns $\mtx{C} \in \mathbb{R}^{m \times \l}$ of the matrix $\mtx{A}$, such that 
    \begin{align*}
        \|\mtx{A} - \mtx{CC^\dagger A R^\dagger R}\|_F &\leq \sqrt{2+2\l} \|\mtx{A} - \mtx{Z}\|_F,\\
        \|\mtx{A} - \mtx{CC^\dagger A R^\dagger R}\|_2 &\leq \sqrt{2+2\l(\min (m,n)-\l)} \|\mtx{A} - \mtx{Z}\|_2.
    \end{align*}
    In the same number of operations it is also possible to select the same rows $\mtx{R} \in \mathbb{R}^{\l \times n}$ but mayber different columns $\mtx{C} \in \mathbb{R}^{m \times \l}$, such that
    \begin{align*}
        \|\mtx{A} - \mtx{C M^\dagger R}\|_F &\leq (\l+1) \|\mtx{A}-\mtx{Z}\|_2,\\
        \|\mtx{A} - \mtx{C M^\dagger R}\|_2 &\leq \sqrt{1+\l(\l+2)(\min(m,n)-\l)} \|\mtx{A}-\mtx{Z}\|_2,
    \end{align*}
    where $\mtx{M} \in \mathbb{R}^{\l \times \l}$ is the submatrix at the intersection of rows $\mtx{R}$ and columns $\mtx{C}$.
\end{theorem}

\begin{corollary}[\cite{osinsky2023close,zamarashkin2018existence}]
    Using $\mtx{Z}=\mtx{A_\l}$, where $\mtx{A_\l}$ is a rank-$\l$ truncated SVD of $\mtx{A}$, we get
    \begin{align*}
        \|\mtx{A} - \mtx{CM^\dagger R}\|_F \leq (\l+1)\|\mtx{A} - \mtx{A_\l}\|_F.
    \end{align*}
\end{corollary}

Standard CUR approximation often monitors the Frobenius norm to reduce aggregate approximation error, due to its unbiasedness and lower variance~\cite{horesh2025variance}.


\subsubsection{Choice of target rank}

Choosing the target rank $\l$ is crucial for the quality and efficiency of the preconditioner. A target rank that is too large can cause numerical instability in LUPP or pseudoinverse computations and increase computational cost, undermining the purpose of low-rank preconditioning; if it is too small, the best rank-$\l$ approximation error, $\sigma_{\l+1}(\mtx{A})$, may be large, preventing accurate approximation. Many works set the target rank of a low-rank approximation proportional to the effective dimension \cite{frangella2023randomized} or statistical rank of $\mtx{A}$, but in practice, these metrics are typically unknown. Thereby, we adopt two adaptive strategies for selecting $\l$ in the CUR approximation.

The fast rank estimation method of \cite{meier2024fast} estimates the numerical rank by repeatedly sketching the matrix from both sides and performing an SVD on the resulting compressed matrix. In particular, Gaussian or SRTT sketches are used to approximate the singular values, from which the rank is inferred (see Algorithm~\ref{alg:cur_rankest}). The total complexity is $\mathcal{O}((m+\log n)n\l)=\mathcal{O}(mn\l)$, where the Gaussian sketch costs $\mathcal{O}(mn \l)$, the SRTT sketch costs $\mathcal{O}(n \l \log n + \l^3)$, and the SVD costs $\mathcal{O}(\l^3)$. In practice, these sketches can be appended rather than recomputed at each iteration, and the final sketch can be reused for the subsequent randomized CUR approximation, so the overall cost remains modest. However, when the estimated rank $\l$ is large, the SVD of the sketched matrix of size $\l \times 2\l$ may become a computational bottleneck.

As an alternative, Pritchard \textit{et al.}~\cite{pritchard2025fast} propose \emph{IterativeCUR}, a fast rank-adaptive CUR approximation method (outlined in Algorithm~\ref{alg:cur_icur}) that requires only a single sketch $\mtx{S}\mtx{A}$, independent of the target rank. The method incrementally increases the CUR rank by selecting additional column and row indices based on the sketched residual $\mtx{S}\mtx{A} - \mtx{S}\mtx{C}\mtx{U}\mtx{R}$. Crucially, the initial sketch $\mtx{S}\mtx{A}$ is reused throughout, and products involving $\mtx{S}\mtx{C}$ are extracted from it, avoiding any additional sketching.
The CUR factors are updated iteratively by augmenting the index sets using the procedure described in Algorithm~\ref{alg:cur_augment}. This results in an efficient rank-adaptive scheme in which the approximation is refined progressively while maintaining low computational cost.


\begin{algorithm}
    \caption{Fast rank estimation \cite{meier2024fast}}
    \label{alg:cur_rankest}
    \begin{algorithmic}[1]
        \Require $\mtx{A} \in \F^{m \times n}$; rank-tolerance $\varepsilon_{\text{rank}}$; initial rank upper-bound estimate $\l_0$.
        \Ensure Estimated rank $\l$.
        \Statex
        \While{true}
        \State $\mtx{S_1} \gets \texttt{sparsesign}(\l_0, m, 8)$ \Comment{$\l_0 \times m$ 
        sparse sign embedding with $\xi = 8$}
        \State $\mtx{X} \gets \mtx{S_1}\mtx{A}$
        \State $\mtx{S_2} \gets \texttt{SRTT}(2\l_0, n)$ \Comment{$2\l_0 \times m$ SRTT embedding}
        \State $[\sigma_1, \ldots, \sigma_{\l_0}] \gets \texttt{svd}(\mtx{X}\mtx{S_2}^\top)$
        \If{$\exists\, \hat{\l}\ \text{s.t.}\ \sigma_{\hat{\l}+1} \le \varepsilon_{\text{rank}} \cdot \sigma_{1}$}
            \State $\l \gets \hat{\l}$ \Comment{estimated $\varepsilon_{\text{rank}}$-rank of $\mtx{A}$}
            \State \texttt{break}
        \Else
            \State $\l_0 \gets 2\l_0$ \Comment{increase rank upper-bound and repeat}
        \EndIf
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{IterativeCUR \cite{pritchard2025fast}}
    \label{alg:cur_icur}
    \begin{algorithmic}[1]
        \Require{$\mtx{A} \in \F^{m \times n}$; block size $\l_0$ (usually in $[5,250]$); error tolerance $\varepsilon_{\text{cur}}$.}
        
        \Statex
        \State $\vct{I} = \vct{J} = \emptyset,\quad \mtx{C}=\mtx{U}=\mtx{R}=\emptyset$
        \State $\mtx{S} \gets \texttt{sparsesign}(1.1\l_0, m, 8)$ \Comment{oversampling}
        \State $\mtx{E}^\textrm{row} \gets \mtx{SA}$ \Comment{sketch once and reuse it}
        \Repeat \Comment{rank grows by $\l_0$ per iteration}
            \State $[\vct{I}, \vct{J}] \gets \texttt{augmentCUR}(\mtx{A}, \mtx{C}, \mtx{U}, \mtx{R}, \mtx{E}, \vct{I}, \vct{J})$ \Comment{use \cref{alg:cur_augment}}
            \State $\mtx{U} \gets \mtx{A(\vct{I}, \vct{J})}^\dagger$
            \Comment{default QR, improved efficiency with LU}
            \State $\mtx{C} \gets \mtx{A}(:, \vct{J})$, $\mtx{R} \gets \mtx{A}(\vct{I},:)$
            \State $\mtx{E}^\textrm{row} \gets \mtx{SA} - \mtx{S C U R}$
            \Comment{Use $\mtx{SC}$ from $\mtx{SA}$}
            \State $\rho \gets \|\mtx{E}^\textrm{row}\|_F / \|\mtx{SA}\|_F$
        \Until{$\rho \leq \varepsilon_{cur}$}
        \Statex
        \State \Return $\mtx{C}, \mtx{U}, \mtx{R}$ \Comment{CUR approximation with rank $\l_0 \times$(\#iterations)}
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{\texttt{augmentCUR}}
    \label{alg:cur_augment}
    \begin{algorithmic}[1]
        \Require Matrix $\mtx{A} \in \F^{m \times n}$; CUR approximation $\mtx{C},\ \mtx{U},\ \mtx{R}$; row-sketched CUR residual $\mtx{E}^\textrm{row} \in \F^{\l_0 \times n}$; current row and column index sets $\vct{I}$ and $\vct{J}$.
        \Ensure $\l = \texttt{size}(\mtx{C},2)$ previous approximation rank
        
        \Statex
        \State $\mtx{E}^\textrm{row}(:,\vct{J})\gets \mtx{0}$ \Comment{avoid reselecting previously chosen indices}
        \State $[\sim, \sim, \vct{P}_\textrm{col}] \gets \texttt{lu}({\mtx{E}^\textrm{row}}^\top, \texttt{`vector'})$ \Comment{default LUPP, can use CPQR or Osinsky}
        \State $\vct{J_+} \gets \vct{P}_\textrm{col}(1:\l_0)$
        \State $\vct{J} \gets [\vct{J}, \vct{J_+}]$
        \Statex
        \State $\mtx{E}^\textrm{col} \gets \mtx{A}(:,\vct{J_+}) - \mtx{CUR}(:, \vct{J_+})$
        \State $\mtx{E}^\textrm{col}(\vct{I},:)\gets \mtx{0}$ \Comment{avoid reselecting previously chosen indices}
        \State $[\sim, \sim, \vct{P}_\textrm{row}] \gets \texttt{lu}(\mtx{E}^\textrm{col}, \texttt{`vector'})$\Comment{default LUPP, can use CPQR or Osinsky}
        \State $\vct{I_+} \gets \vct{P}_\textrm{row}(1:\l_0)$
        \State $\vct{I} \gets [\vct{I}, \vct{I_+}]$

        \Statex
        \State \Return $\vct{I},\ \vct{J}$
        \Comment{$\l_0$ additional row and column indices}
    \end{algorithmic}
\end{algorithm}

\subsection{Implementation and complexity}
\subsubsection{Supplementary Algorithms}

\cref{sec:svdfreepreconditioner}

\begin{algorithm}[H]
    \caption{\texttt{SVD-free CURPreconditioner}}
    \label{alg:svdfreepreconditioner}
    \begin{algorithmic}[1]
        \Require{Matrix $\mtx{A}$, row and column indices $\mtx{I}$ and $\vct{J}$, regularization parameter $\mu$.}
        \Ensure Preconditioner inverse operator $\mtx{\widetilde{P}}^{-1}$

        \State $\mtx{C} \gets \mtx{A}(:, \vct{J})$
        \State $\mtx{R} \gets \mtx{A}(\vct{I},:)$
        \Statex
        \State \textbf{Part 1: Factorize $\mtx{C}$ and $\mtx{R}$}
        \State $\mtx{T_C} \gets \texttt{chol}(\mtx{C}^\top \mtx{C})$\Comment{sketched Cholesky QR for stability}
        \State $[\mtx{Q_R}, \mtx{T_R}] \gets \texttt{qr}(\mtx{R^\top})$
        \Comment{sketched Cholesky QR for efficiency}
        
        \Statex
        \State \textbf{Part 2: Build spectral preconditioning operator}
        \State $\mtx{M}^{-1} \gets \mtx{T_R}^{-\top}\mtx{A}(\vct{I},\vct{J}) \mtx{T_C}^{-1}$ 
        \State $\svhat \gets $ estimate of CUR spectral error by \cref{eq:2normestimate} \Comment{target level}
        \State $\mtx{\tilde{P}}^{-1} \gets \svhat\mtx{Q_R} \mtx{M}^{-1}\mtx{Q_R}^\top + (\mtx{I_n}-\mtx{Q_R Q_R^\top})$
        \Comment{apply via \texttt{matvec}}
    \end{algorithmic}
\end{algorithm}

For efficient updates of QR factorization, we use \cref{alg:augmentqr}.

\begin{algorithm}[H]
    \caption{\texttt{augmentQR}}
    \label{alg:augmentqr}
    \begin{algorithmic}[1]
        \Require Orthonormal $\mtx{Q}\in\F^{m\times n}$, upper-triangular $\mtx{R}\in\F^{n\times n}$, additional columns $\mtx{C}\in\F^{m\times p}$
        \Ensure Orthonormal $\mtx{Q}_{\mathrm{new}}\in\F^{m\times(n+p)}$ and upper-triangular $\mtx{R}_{\mathrm{new}}\in\F^{(n+p)\times(n+p)}$ with $[\mtx{Q}_{\mathrm{new}}, \mtx{R}_{\mathrm{new}}]=\texttt{qr}([\mtx{Q}\mtx{R},\mtx{C}])$
        \Statex
        \State $\mtx{P}_1 \gets \mtx{Q}^\top \mtx{C}$
        \State $\mtx{E} \gets \mtx{C} - \mtx{Q}\mtx{P}_1$ \Comment{project and form residual}
        \State $\mtx{P}_2 \gets \mtx{Q}^\top \mtx{E}$ \Comment{re-orthogonalization (optional but recommended)}
        \State $\mtx{E} \gets \mtx{E} - \mtx{Q}\mtx{P}_2$
        \State $[\mtx{Q_E}, \mtx{R_E}] \gets \texttt{qr}(\mtx{E},0)$ \Comment{sketched Cholesky QR can be used}
        \State $\mtx{Q}_{\mathrm{new}} \gets [\mtx{Q},\ \mtx{Q_E}]$
        \State $\mtx{R}_{\mathrm{new}} \gets \begin{bmatrix} \mtx{R} & \mtx{P}_1+\mtx{P}_2 \\[2pt] \mtx{0} & \mtx{R_E} \end{bmatrix}$
        \Statex
        \State \Return $\mtx{Q}_{\mathrm{new}},\ \mtx{R}_{\mathrm{new}}$
    \end{algorithmic}
\end{algorithm}
\subsubsection{Detailed computational complexity}\label{app:complexity}

The computational cost of the proposed algorithm is dominated by two primary components: (i) factorizations associated with constructing and updating the low-rank preconditioner, and (ii) matrix–matrix multiplications involving the full problem dimensions $m$ and $n$. We detail each below, emphasising how these costs are mitigated in practice.

\paragraph{Preconditioner construction}
Given CUR factors, constructing a rank-$\ell$ preconditioner costs $\mathcal{O}((m+n+\ell)\ell^2)$, while both storage and application cost $\mathcal{O}(n\ell)$.

\paragraph{Factorization costs}

A dominant cost arises in each preconditioning update (\cref{alg:preconditioner}, line~5), where an SVD of a dense $\l \times \l$ matrix is required. This step costs $\mathcal{O}(\l^3)$ and is typically the most expensive operation. The SVD-free variant introduced in \cref{sec:svdfreepreconditioner} eliminates this decomposition entirely, reducing the construction cost by $\mathcal{O}(\l^3)$ (with large constant). The trade-off is a modest increase in application cost: applying the preconditioner requires two additional triangular solves, contributing approximately $2\l^2$ extra flops per iteration.

Maintaining a QR factorization of the growing matrix $\mtx{R}^\top \in \F^{n \times q\l_0}$ (with $q = \l/\l_0$) would naively cost $\mathcal{O}(n\l^3/\l_0)$. Instead, we update the factorization incrementally using \cref{alg:augmentqr}, reducing the cost to $\mathcal{O}(n\l^2)$. In addition, we employ a block QR append strategy together with a sketched Cholesky QR, which improves efficiency while maintaining numerical stability.

The pseudoinverse of the CUR core matrix introduces another factorization cost. A direct QR-based approach leads to $\mathcal{O}(\l^4)$ complexity. While update techniques based on Givens rotations can reduce this to $\mathcal{O}(\l^3/\l_0)$, in practice we instead exploit highly optimised dense factorizations. In particular, replacing QR with LU can improve performance due to better parallel scalability, while remaining sufficiently accurate for moderately conditioned problems.

Finally, LUPP factorizations required in the CUR construction incur a cost of $\mathcal{O}(\l\l_0(m+n))$.

\paragraph{Matrix–matrix multiplications.}

Matrix–matrix multiplications involving the full dimensions $m$ and $n$ arise in several parts of the algorithm. In particular, the computation of column and row residuals during CUR updates involves products with nominal complexity $\mathcal{O}((m+n)\l^2)$. These operations are implemented as BLAS-3 kernels and therefore achieve high efficiency on modern hardware. When $\mtx{C}$ and $\mtx{R}$ are sparse, the effective cost is substantially reduced.

In forming and applying the preconditioner, we avoid explicitly constructing large dense intermediate matrices. For example, products of the form $\mtx{Q_R}\Vhat_M$ are applied implicitly via matrix–vector operations. When $\mtx{R}$ is sparse, we further exploit the representation $\mtx{R}\mtx{T_R^{-1}}$ to reduce both computational and storage costs.

\paragraph{Sketching and additional costs.}

The initial sketching step (\cref{alg:aplls}, lines~3--4) can be expensive for large $m$ and $n$. A Gaussian sketch requires $\mathcal{O}(mn\l_0)$ operations and is therefore impractical at scale. To mitigate this, we employ sparse sign embeddings~\cite{nelson2013osnap, cohen2016nearly}, reducing the cost to $\mathcal{O}(\xi \cdot \mathrm{nnz}(\mtx{A}))$, where $\xi$ is the number of nonzeros per column of the sketching matrix (typically $\xi = \min(\l_0, 8)$~\cite{tropp2019streaming}).

Additional costs include residual norm evaluation for convergence monitoring, which requires $\mathcal{O}(n\l_0)$ operations and is negligible compared to the dominant terms above.

\subsubsection{Practical factorisation choices}
% QR vs LU, SVD-free variant, incremental QR updates.



\subsection{Numerical Studies}\label{app:numericalstudies_detail}

This section contains the technical details required for an efficient implementation, including detailed explanation of the interplay between spectral structure and Krylov convergence, sketch choices, and hyperparameter choices.

\subsubsection{Overpreconditioning}\label{sec:overpreconditioning_detail}
Consider a matrix $\mtx{A}$ whose singular values satisfy $\sigma_1 \geq  \cdots \geq \sigma_\l \gg \sigma_{\l+1} \geq \cdots \sigma_n$. A rank-$k$ spectral preconditioner with $k = \l$ collapses the dominant singular values to the level $\hat{\sigma}=\sigma_{\l}$, hence still preserving a clear separation from trailing singular values $\sigma_{\ell+1},\ldots,\sigma_n$. In contrast, when $k > \l$, the target level $\hat{\sigma}=\sigma_k$ lies within the cluster of trailing singular values, destroying the spectral separation between dominant and trailing components. 

This spectral gap is precisely what allows LSQR to distinguish between directions that are already effectively resolved and those that still require correction. Indeed, LSQR builds Krylov subspaces of the form $$\mathcal{K}_j(\widetilde{\mtx{A}}^\top\widetilde{\mtx{A}}, \widetilde{\mtx{A}}^\top \vct{b}), \quad \widetilde{\mtx{A}}^\top \vct{b} = \widetilde{\mtx{V}}\widetilde{\mtx{\Sigma}}\widetilde{\mtx{U}}^\top \vct{b},$$ so early Krylov bases are dominated by singular directions corresponding to large values of $\widetilde\sigma_i \widetilde{\vct{u}}_i^\top \vct{b}$. A clear spectral gap allows Krylov polynomials to selectively resolve these dominant components.

When the spectral gap is destroyed by over-preconditioning ($k > \l$), the singular values of the preconditioned matrix become tightly clustered. As a result, singular directions are no longer well separated spectrally, Ritz vectors mix dominant and trailing components, and Krylov polynomial filtering becomes ineffective.  (small perturbations can easily roate singular vectors)

In problems where the transformed solution $\vct{y}\ast=\mtx{P}\vct{x}\ast$ is approximately uniformly distributed across singular directions (e.g., inconsistent or consistent-b settings), convergence is then driven primarily by the reduced condition number and is less sensitive to the precise alignment of early Krylov bases. In contrast, in consistent-$x$ settings where $\vct{y}_\ast$ is strongly biased toward the dominant right singular subspace of the original matrix, the misalignment between early Krylov bases and these dominant directions leads to inefficient convergence despite improved conditioning.

This analysis explains why over-preconditioning can be counterproductive and directly motivates an adaptive strategy that alternates between progressive preconditioning and LSQR phases. In the early LSQR phases, the solution is sought on a preconditioned problem that retains sufficient spectral separation to enable efficient resolution of the dominant components. In later phases, LSQR is warm-started using the driving vector $\widetilde{\mtx{A}}^\top(\vct{b}-\widetilde{\mtx{A}}\vct{y_0})$, at which point the presence of a pronounced spectral gap is no longer essential, as the residual is confined to a progressively refined subspaced. Moreover, the adaptive CUR approximation inherently prevents overestimation of the target rank, ensuring that additional preconditioning effort is introduced only when it is likely to be beneficial.


\subsubsection{Different sketches}\label{sec:sketch}
We are also motivated to study the impact of different sketching types. In this set of experiments, we consider three sketch types: Gaussian embeddings, sparse embeddings with $\xi=8$~\cite{kane2014sparser}, and SRFT (or 1-hashing embeddings~\cite{cartis2021hashing}), all with sketch dimension $s$. \cref{table:sketchcost} summarises the asymptotic cost of applying the different sketching operators. For Gaussian and sparse embeddings, the cost scales linearly with the number of nonzeros in $A$. In contrast, the SRFT embedding relies on a dense orthogonal transform, resulting in a cost that scales with the full matrix dimensions.
\jh{experiments on sparse matrices}
\input{plot_tex/num_stud_sketch}

\begin{table}[t]
\centering
\caption{Asymptotic cost of applying different sketching matrices to an $m \times n$ matrix $A$.
Here $s$ denotes the sketch dimension, $\xi$ the number of nonzeros per column in the sparse embedding,
and $\mathrm{nnz}(A)$ the number of nonzero entries in $A$.}
\label{table:sketchcost}
\begin{tabular}{lc}
\toprule
Sketch type & Cost \\ 
\midrule
Gaussian embedding 
& $\mathcal{O}\!\left(s\,\mathrm{nnz}(A)\right)$ \\

Sparse embedding 
& $\mathcal{O}\!\left(\xi\,\mathrm{nnz}(A)\right)$ \\

SRFT\footnotemark 
& $\mathcal{O}\!\left(m n \log m\right)$ \\
\bottomrule
\end{tabular}
\end{table}
\footnotetext{The stated cost for the SRFT embedding assumes a standard fast transform
(e.g. DCT or Hadamard), which densifies the input matrix.} 


\jh{The blocksize $\l_0$ here is playing a big role throughout the algorithm. Pritchard et al.~\cite{pritchard2025fast} shows that empirically the high approximation accuracy is preserved even block sizes as small as five, but for optimal computational speed, larger block sizes (around 100) perform better. ~\cite{pritchard2025fast}, choice of target level $\svhat$.}

\subsubsection{Hyperparameters for adaptivity}

The behavior of the fully adaptive scheme is controlled by three hyperparameters: the CUR error tolerance $\varepsilon_{cur}$, the re-preconditioning tolerance $\nu_{prec}$, and the dynamic LSQR stopping tolerance $\nu_{lsqr}$. Together, these regulate rank growth, preconditioner updates, and the balance between preconditioning and Krylov iterations.


% \paragraph{CUR error tolerance}

From \cref{sec:adaptiveprec_sensitivity}, we see that our method is robust to moderate overestimation of the target rank but sensitive to underestimation. Consequently, the CUR tolerance $\varepsilon_{cur}$ must be chosen to avoid truncating significant spectral components.
For regularized problems, the regularization parameter $\mu$ provides a natural reference as it determines the desired solution accuracy. Accordingly, we set 
\[
\varepsilon_{cur} \propto \mu,
\]
and study its effect on rank selection and convergence. The resulting behavior shows that early convergence is largely insensitive to the tolerance, whereas overly small tolerances trigger unnecessary rank growth and increase runtime with negligible residual improvement. Hence, we recommend $\varepsilon_{cur} \in [30\mu, 100\mu]$.

% \subsubsection{Studies on CUR approximation hyperparameters}\label{sec:cur_errtol}
% In this section, we investigate suitable choices of CUR approximation error tolerance that lead to an appropriate target rank.

% Since the regularization parameter $\mu$ is closely related to the desired solution accuracy, we set the error tolerance to be proportional to $\mu$. Specifically, we vary the base tolerance $\varepsilon_{cur}$ over values $\mu, 3\mu, 10\mu, 30\mu$, and $100\mu$. Figure~\ref{fig:num_stud_errtol} presents representative example. Since the error tolerance primarily determines the number of CUR refinement iterations, the initial behavior of the algorithm is constructively identical across tolerances, and the early convergence of LSQR is therefore unaffected. However, for smaller tolerances, the target rank is overestimated, leading to unnecesary re-preconditioning phases that dominate the overall computational cost.

% An additional observation is that LSQR convergence is not governed solely by the condition number of the preconditioned system. As shown in Figure~\ref{fig:num_stud_errtol}(c), for base tolerances of $30\mu$ and $100\mu$, the leading singular values of the preconditioned matrix remain on the order of $10^{2}$, in contrast to the other cases where they are clustered near $10^{-5}$. Nevertheless, Figure~\ref{fig:num_stud_errtol}(b) shows that the corresponding residual convergence is comparable, and in some cases faster, such as for the $30\mu$ tolerance. This behavior illustrates that LSQR convergence is more closely correlated with the clustering of singular values than with the overall condition number of the preconditioned matrix.

% \input{plot_tex/num_stud_errtol}

% \paragraph{Schedule adaptivity}

The balance between preconditioning and LSQR solving phases is controlled through the choice of re-preconditioning tolerance $\nu_{prec}$ and LSQR dynamic stopping tolerance $\nu_{prec}$, as defined in \cref{sec:adaptivitycriteria}.
The re-preconditioning tolerance $\nu_{\mathrm{prec}}$ controls when the preconditioner is updated. Since constructing the preconditioner $\mtx{P}$ is relatively expensive, updates should be triggered only when a meaningful improvement in preconditioning quality is expected, unless we use the SVD-free variant. In practice, performance is largely insensitive to the exact choice of $\nu_{\mathrm{prec}}$, and a moderate value (e.g.\ $\nu_{\mathrm{prec}} = 10$) provides a good balance between avoiding unnecessary updates and maintaining effective preconditioning.

% \cref{fig:num_stud_errdist} illustrates the effect of the re-preconditioning tolerance $\nu_{\mathrm{prec}}$ on convergence behaviour. Smaller values lead to faster initial progress but trigger frequent preconditioner reconstructions, which increase the overall runtime. Larger values reduce redundant re-preconditioning at the cost of slower early convergence. In practice, a moderate tolerance (e.g. $\nu_{\mathrm{prec}} = 10$) provides a good balance between early convergence and total time to solution.
% \jh{Get rid of the plot. Just say it is largely invariant to err\_dist, so we empirically just suggest err\_dist of 10.}

% \input{plot_tex/num_stud_errdist}

The LSQR tolerance $\nu_{\mathrm{lsqr}}$ determines when intermediate LSQR phases terminate. If $\nu_{\mathrm{lsqr}}$ is too small, LSQR may terminate prematurely despite strong convergence, leading to overly frequent re-preconditioning and increased total runtime. Conversely, if $\nu_{\mathrm{lsqr}}$ is too large, LSQR may continue despite slow progress, resulting in wasted iterations. Empirically, values in the range $\nu_{\mathrm{lsqr}} \in [100, 200]$ provide a good trade-off, as illustrated in \cref{fig:num_stud_cvgrate}.

Warm-starting LSQR after each preconditioner update preserves continuity across phases and helps mitigate degradation due to over-preconditioning, but its effectiveness depends on the choice of $\nu_{\mathrm{lsqr}}$. If LSQR phases terminate too early, over-preconditioning may destroy the spectral gap before a sufficiently accurate solution is reached, leading to slow convergence in the final LSQR phase (see \cref{sec:overpreconditioning}).

\input{plot_tex/num_stud_cvgrate}

\subsubsection{Benchmarking Experiments}\label{app:benchmark_general}
\input{plot_tex/appendix_restimes}

\mainalg{} is not always the fastest method to reach a specific tolerance, it consistently delivers stable and competitive performance across the entire time horizon. 


==> plot_tex/num_stud_errdist.tex <==

\begin{figure}[!htbp]
  \centering

  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errdists/restime d_6k5k_i_coh.png}
    \caption{Residuals vs. Time}
  \end{subfigure}\hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errdists/restime d_15k2k_sm_i_coh.png}
    \caption{Residuals vs. Time}
  \end{subfigure}\hfill
  
  \caption{Effect of the re-preconditioning tolerance $\nu_{\mathrm{prec}}$ (values 2, 10, and 50). Smaller tolerances yield faster early convergence but incur more frequent preconditioner updates, while larger tolerances reduce redundant updates at the expense of slower initial progress.}
  \label{fig:num_stud_errdist}
\end{figure}

==> plot_tex/num_stud_errtol.tex <==
%% Experiment 134 Results

%% Dense 6k5k
\begin{figure}[!htbp]
  \centering

  \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errtols2/restime d_6k5k_x_coh.pdf}
    \caption{\centering Sharp decay\\consistent-x}
  \end{subfigure}\hfill
  %
  \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errtols2/restime d_6k5k_sm_x_coh.pdf}
    \caption{\centering Smooth decay\\consistent-x}
  \end{subfigure}\hfill
  %
  \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errtols2/restime d_6k5k_b_coh.pdf}
    \caption{\centering Sharp decay\\consistent-b}
  \end{subfigure}\hfill
  %
  \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.28\textheight,keepaspectratio]
      {restimes8_errtols2/restime d_6k5k_sm_b_coh.pdf}
    \caption{\centering Smooth decay\\consistent-b}
  \end{subfigure}\hfill
  
  \caption{Effect of CUR approximation error tolerance on convergence and preconditioning quality. The base tolerance $\varepsilon_{\mathrm{cur}}$ is varied over ${\mu,10\mu,50\mu,100\mu,500\mu}$.}
  \label{fig:num_stud_errtol}
\end{figure}



==> table.tex <==
\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{3} & 12 & 27 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 17 & 21 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 250 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{10} & 143 & 24 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{9} & 13 & 23 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 65 & 63 & \textbf{3} & 5 & 21 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 67 & 70 & \textbf{2} & 3 & 22 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 143 & 133 & 23 & \textbf{11} & 18 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 148 & 159 & 28 & \textbf{15} & 22 \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = d, consistency = x}
\end{table}


\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 15 & 13 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 19 & 12 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 250 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & 9 & 68 & \textbf{7} \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{8} & 17 & 19 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 82 & 71 & \textbf{3} & \textbf{3} & 7 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 77 & 86 & 5 & \textbf{4} & 11 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 154 & 184 & 29 & \textbf{5} & 9 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 189 & 203 & 32 & 19 & \textbf{13} \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = d, consistency = b}
\end{table}


\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 15 & 14 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 21 & 13 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 250 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{8} & 96 & 10 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{9} & 20 & 14 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 85 & 74 & \textbf{2} & 4 & 9 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 79 & 87 & 5 & \textbf{3} & 12 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 170 & 144 & 29 & \textbf{6} & 10 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 178 & 166 & 30 & 23 & \textbf{9} \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = d, consistency = i}
\end{table}


\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{16} & 18 & 35 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{6} & 17 & 25 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{4} & 19 & 23 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 6 & 24 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 54 & 58 & \textbf{2} & 3 & 22 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 65 & 65 & \textbf{2} & 4 & 20 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 149 & 147 & 21 & \textbf{11} & 20 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 127 & 125 & 19 & \textbf{11} & 15 \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = sp1e-02, consistency = x}
\end{table}


\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & 22 & \textbf{14} & \textbf{14} \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{6} & 24 & 18 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{8} & 19 & 9 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 15 & 11 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 78 & 74 & 5 & \textbf{3} & 13 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 76 & 66 & 5 & \textbf{3} & 6 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 164 & 169 & 27 & 26 & \textbf{5} \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 146 & 157 & 28 & 21 & \textbf{7} \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = sp1e-02, consistency = b}
\end{table}


\begin{table}\begin{tabular}{|l|l|l|l|c|c|c|c|c|}
\hline
Size & Decay & Coh & Metric & cg & lsqr & npcg & icurlsqr & bdplsqr \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & 23 & 26 & \textbf{13} \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 80 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{6} & 24 & 15 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{9} & 21 & 10 \\
\hline
\multirow{2}{*}{600 $\times$ 500} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & 160 & \textbf{20} & 1100 \\
 & & & Iters & 501 & 501 & \textbf{2} & 15 & 9 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 74 & 74 & \textbf{3} & \textbf{3} & 8 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{sharp} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 66 & 80 & \textbf{3} & 4 & 7 \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{incoh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 172 & 171 & 32 & 26 & \textbf{13} \\
\hline
\multirow{2}{*}{6000 $\times$ 100} & \multirow{2}{*}{smooth} & \multirow{2}{*}{coh} & SketchSize & 0 & 0 & \textbf{20} & \textbf{20} & 300 \\
 & & & Iters & 157 & 172 & 28 & 24 & \textbf{6} \\
\hline
\hline
\end{tabular}
\caption{Results for sparsity = sp1e-02, consistency = i}
\end{table}



